TANDEM: Tracking and Dense Mapping in Real-time using Deep Multi-view Stereo

In this paper, we present TANDEM a real-time monocular tracking and dense mapping framework. For pose estimation, TANDEM performs photometric bundle adjustment based on a sliding window of keyframes. To increase the robustness, we propose a novel tracking front-end that performs dense direct image alignment using depth maps rendered from a global model that is built incrementally from dense depth predictions. To predict the dense depth maps, we propose Cascade View-Aggregation MVSNet (CVA-MVSNet) that utilizes the entire active keyframe window by hierarchically constructing 3D cost volumes with adaptive view aggregation to balance the different stereo baselines between the keyframes. Finally, the predicted depth maps are fused into a consistent global map represented as a truncated signed distance function (TSDF) voxel grid. Our experimental results show that TANDEM outperforms other state-of-the-art traditional and learning-based monocular visual odometry (VO) methods in terms of camera tracking. Moreover, TANDEM shows state-of-the-art real-time 3D reconstruction performance.

==> backup_figs.tex <==
\begin{figure}[tb]
  \centering
    \includegraphics[width=3.4in]{figures/traj_comp_plasma.eps}
\caption{\nan{Consider to remove this fugure from the main paper if no enough space. }Estimated trajectories of DeepFactors and TANDEM on icl/office1. For both methods we select the run with the median error (cf. \autoref{tab:trajectory_eval}).}
  \label{fig:traj_comp}
  \vspace{-0.5cm}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=3.4in]{figures/tracking_dist.eps}
  \caption{Trajectory evaluation on the ICL-NUIM dataset. Because all systems use monocular images we perform $\text{Sim}(3)$ alignment w.r.t. the ground truth trajectory. We show the color-coded absolute trajectory error (ATE) for five runs. The results show that our dense tracking improves the robustness over our baseline system. DeepFactors produces nearly identical results for all five runs, but the median error is higher than for the proposed system.}
  \label{fig:trajectory_eval}
\end{figure}

\begin{figure}[tb]
  \centering
    \includegraphics[width=0.7\textwidth]{figures/tracking_euroc_boxplot.pdf}
\caption{Tracking result for the EuRoC dataset.}
 \label{fig:timing}
